Mol-Instructions: A Large-Scale Biomolecular Instruction Dataset for Large Language Models

Large Language Models (LLMs), with their remarkable task-handling capabilities and innovative outputs, have catalyzed significant advancements across a spectrum of fields. However, their proficiency within specialized domains such as biomolecular studies remains limited. To address this challenge, we introduce Mol-Instructions, a comprehensive instruction dataset designed for the biomolecular domain. Mol-Instructions encompasses three key components: molecule-oriented instructions, protein-oriented instructions, and biomolecular text instructions. Each component aims to improve the understanding and prediction capabilities of LLMs concerning biomolecular features and behaviors. Through extensive instruction tuning experiments on LLMs, we demonstrate the effectiveness of Mol-Instructions in enhancing large models' performance in the intricate realm of biomolecular studies, thus fostering progress in the biomolecular research community. Mol-Instructions is publicly available for ongoing research and will undergo regular updates to enhance its applicability.

==> tables/biotext.tex <==
\begin{table*}[!t]
\vskip -0.1in
\centering
\small
\caption{\small
Results for NLP tasks in bioinformatic domain. (C)ER denotes chemical entity recognition, (C-D)IE signifies chemical-disease interaction extraction, and (C-P)IE stands for chemical-protein interaction extraction.
}
\vskip 0.1in
\scalebox{0.8}{
\begin{tabular}{lcccccccc}
\toprule
{\multirow{3}{*}{\textsc{Model}}} 
& \multicolumn{1}{c}{\textsc{True or False}}
& \multicolumn{3}{c}{\textsc{Open Question}} 
& \multicolumn{1}{c}{\textsc{Multi-choice}}
& \multicolumn{1}{c}{\textsc{(C)ER}}
& \multicolumn{1}{c}{\textsc{(C-D)IE}}
& \multicolumn{1}{c}{\textsc{(C-P)IE}}
\\
\cmidrule(lr){2-2}
\cmidrule(lr){3-5}
\cmidrule(lr){6-6}
\cmidrule(lr){7-7}
\cmidrule(lr){8-8}
\cmidrule(lr){9-9}
& \textsc{Acc} $\uparrow$  & \textsc{BLEU} $\uparrow$  & \textsc{ROUGE-1} $\uparrow$  & \textsc{BertScore} $\uparrow$ & \textsc{Acc} $\uparrow$ & \textsc{F1} $\uparrow$ & \textsc{F1} $\uparrow$ & \textsc{F1} $\uparrow$\\
\midrule 
\textsc{Alpaca} & 0.33 & 0.0027 & 0.0880 & 0.8237 & 0.286 & 0.21 & 0.04 & 0.002 \\
\textsc{Baize} &  0.48 & 0.0051 & 0.1003 & 0.8114 & 0.237 & 0.01 & 0.004 & 0.004 \\
\textsc{ChatGLM} & 0.18 & 0.0029 & 0.0904 & 0.7952 & 0.223 & 0.15 & 0.02 & 0.002 \\
\textsc{LLama} & 0.27 & 0.0033 & 0.0999 & 0.8136 & 0.297 & 0.00 & 0.05 & 0.003 \\
\textsc{Vicuna} & 0.12 & 0.0043 & 0.0970 & 0.8141 & 0.290 & 0.02 & 0.084 & 0.013 \\
\midrule
\textbf{Ours} & \textbf{0.55} &  \textbf{0.0241} &  \textbf{0.2206} &  \textbf{0.8368} &  \textbf{0.6490} & \textbf{0.75} &  \textbf{0.40} &  \textbf{0.222} \\
\bottomrule
\end{tabular}
}
\vskip -0.15in
\label{tab:res_biotext}
\end{table*}

==> tables/mol_results.tex <==
% \begin{table*}[!b]
% \vskip -0.3in
% \centering
% \small
% \caption{\small
% Results of molecule understanding and property prediction tasks.
% }
% \vskip 0.07in
% \scalebox{0.78}{
% \begin{tabular}{lccccccc}
% \toprule
% {\multirow{3}{*}{\textsc{Model}}} 
% & \multicolumn{6}{c}{\textsc{Molecular Description Generation}}
% & \multicolumn{1}{c}{\textsc{Property Prediction}} \\
% \cmidrule(lr){2-7}
% \cmidrule(lr){8-8}
% &\textsc{BLEU-2} $\uparrow$  & \textsc{BLEU-4} $\uparrow$  & \textsc{ROUGE-1} $\uparrow$  & \textsc{ROUGE-2} $\uparrow$  & \textsc{ROUGE-L} $\uparrow$ & \textsc{METEOR} $\uparrow$ & \textsc{MAE} $\downarrow$ \\
% \midrule 
% \textsc{Alpaca} & 0.068 & 0.014 & 0.178 & 0.041 & 0.136 & 0.107 & 322.109\\
% \textsc{Baize} &  0.064 & 0.015 & 0.189 & 0.053 & 0.148 & 0.106 & 261.343\\
% \textsc{ChatGLM} & 0.055 & 0.011 & 0.163 & 0.036 & 0.121 & 0.105 & - \\
% \textsc{LLama} & 0.059 & 0.014 & 0.164 & 0.066 & 0.148 & 0.184 & 5.553\\
% \textsc{Vicuna} & 0.052 & 0.011 & 0.151 & 0.055 & 0.130 & 0.168 & 860.051 \\
% \midrule
% \textbf{Ours} & \textbf{0.257} &  \textbf{0.219} & \textbf{0.667} &  \textbf{0.588} &  \textbf{0.653} &  \textbf{0.558} &  \textbf{0.013} \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:moldes_prop}
% \end{table*}



% \begin{table*}[!t]
% % \vskip -0.1in
% \centering
% \small
% \caption{\small
% Description-guided molecule design and reagent prediction results.
% }
% \vskip 0.1in
% \scalebox{0.64}{
% \begin{tabular}{l|ccccccc|ccccccc}
% \toprule
% {\multirow{3}{*}{\textbf{Model}}} 
% & \multicolumn{7}{c|}{\textbf{Description-guided Molecule Design}}
% & \multicolumn{7}{c}{\textbf{Reagent Prediction}} \\
% \cmidrule{2-15}
% &Exact$\uparrow$  & BLEU$\uparrow$  & Leven$\downarrow$  & RDK$\uparrow$  & MAC$\uparrow$ & Morgan$\uparrow$ & Validity$\uparrow$ & Exact$\uparrow$  & BLEU$\uparrow$  & Leven$\downarrow$  & RDK$\uparrow$  & MAC$\uparrow$ & Morgan$\uparrow$ & Validity$\uparrow$ \\
% \midrule 
% \textsc{Alpaca} & 0.000 & 0.004 & 51.088 & 0.006 & 0.029 & 0.000 & 0.141 & 0.000 & 0.026 & 29.037 & 0.029 & 0.016 & 0.001 & 0.186 \\
% \textsc{Baize} & 0.000 & 0.006 & 53.796 & 0.000 & 0.000 & 0.000 & 0.151 & 0.000 & 0.051 & 30.628 & 0.022 & 0.018 & 0.004 & 0.099 \\
% \textsc{ChatGLM} & 0.000 & 0.004 & 53.157 & 0.005 & 0.000 & 0.000 & 0.098 & 0.000 & 0.019 & 28.169 & 0.017 & 0.006 & 0.002 & 0.074 \\
% \midrule
% \textbf{Ours} & \textbf{0.001} & \textbf{0.563} & \textbf{40.587} & \textbf{0.219} & \textbf{0.411} & \textbf{0.156} & \textbf{1.000} & \textbf{0.003} & \textbf{0.224} & \textbf{28.519} & \textbf{0.049} & \textbf{0.085} & \textbf{0.023} & \textbf{1.000}\\
% \midrule
% \midrule
% {\multirow{3}{*}{\textbf{Model}}} 
% & \multicolumn{7}{c|}{\textbf{Forward Reaction Prediction}}
% & \multicolumn{7}{c}{\textbf{Retrosynthesis}} \\
% \cmidrule{2-15}
% &Exact$\uparrow$  & BLEU$\uparrow$  & Leven$\downarrow$  & RDK$\uparrow$  & MAC$\uparrow$ & Morgan$\uparrow$ & Validity$\uparrow$ & Exact$\uparrow$  & BLEU$\uparrow$  & Leven$\downarrow$  & RDK$\uparrow$  & MAC$\uparrow$ & Morgan$\uparrow$ & Validity$\uparrow$ \\
% \midrule 
% \textsc{Alpaca} & 0.000 & 0.065 & 41.989 & 0.004 & 0.024 & 0.008 & 0.138 & 0.000 & 0.063 & 46.915 & 0.005 & 0.023 & 0.007 & 0.160 \\
% \textsc{Baize} &  0.000 & 0.044 & 41.500 & 0.004 & 0.025 & 0.009 & 0.097 & 0.000 & 0.095 & 44.714 & 0.025 & 0.050 & 0.023 & 0.112 \\
% \textsc{ChatGLM} & 0.000 & 0.183 & 40.008 & 0.050 & 0.100 & 0.044 & 0.108 & 0.000 & 0.117 & 48.365 & 0.056 & 0.075 & 0.043 & 0.046 \\
% \midrule
% \textbf{Ours} & \textbf{0.018} & \textbf{0.698} & \textbf{30.336} & \textbf{0.252} & \textbf{0.441} & \textbf{0.190} & \textbf{1.000} & \textbf{0.004} & \textbf{0.715} & \textbf{34.196} & \textbf{0.256} & \textbf{0.443} & \textbf{0.195} & \textbf{1.000} \\
% \bottomrule
% \end{tabular}
% }
% \vskip -0.15in
% \label{tab:design_reagent}
% \end{table*}

% \begin{table*}[!t]
% % \vskip -0.1in
% \centering
% \small
% \caption{\small
% Forward reaction and retrosynthesis results.
% }
% \vskip 0.1in
% \scalebox{0.64}{
% \begin{tabular}{l|ccccccc|ccccccc}
% \toprule
% {\multirow{3}{*}{\textbf{Model}}} 
% & \multicolumn{7}{c|}{\textbf{Forward Reaction Prediction}}
% & \multicolumn{7}{c}{\textbf{Retrosynthesis}} \\
% \cmidrule{2-15}
% &Exact$\uparrow$  & BLEU$\uparrow$  & Leven$\downarrow$  & RDK$\uparrow$  & MAC$\uparrow$ & Morgan$\uparrow$ & Validity$\uparrow$ & Exact$\uparrow$  & BLEU$\uparrow$  & Leven$\downarrow$  & RDK$\uparrow$  & MAC$\uparrow$ & Morgan$\uparrow$ & Validity$\uparrow$ \\
% \midrule 
% \textsc{Alpaca} & 0.000 & 0.065 & 41.989 & 0.004 & 0.024 & 0.008 & 0.138 & 0.000 & 0.063 & 46.915 & 0.005 & 0.023 & 0.007 & 0.160 \\
% \textsc{Baize} &  0.000 & 0.044 & 41.500 & 0.004 & 0.025 & 0.009 & 0.097 & 0.000 & 0.095 & 44.714 & 0.025 & 0.050 & 0.023 & 0.112 \\
% \textsc{ChatGLM} & 0.000 & 0.183 & 40.008 & 0.050 & 0.100 & 0.044 & 0.108 & 0.000 & 0.117 & 48.365 & 0.056 & 0.075 & 0.043 & 0.046 \\
% \midrule
% \textbf{Ours} & \textbf{0.018} & \textbf{0.698} & \textbf{30.336} & \textbf{0.252} & \textbf{0.441} & \textbf{0.190} & \textbf{1.000} & \textbf{0.004} & \textbf{0.715} & \textbf{34.196} & \textbf{0.256} & \textbf{0.443} & \textbf{0.195} & \textbf{1.000} \\
% \bottomrule
% \end{tabular}
% }
% \vskip -0.15in
% \label{tab:forward_retro}
% \end{table*}



\begin{table*}[t]
\centering
\vskip 0.05in
\small
\caption{\small
Results of molecular generation tasks. These tasks encompass description-guided molecule design, reagent prediction, forward reaction prediction, and retrosynthesis. \rebut{The symbol $^\clubsuit$ indicates LLMs, while $^\spadesuit$ denotes domain-specific smaller models.}
}
\scalebox{0.75}{
\begin{tabular}{clccccccc}
\toprule
% {\multirow{3}{*}{\textsc{Model}}} 
% & \multicolumn{7}{c}{\textsc{Molecular generation tasks}} \\
% \cmidrule{2-8}
& \textsc{Model}
&\textsc{Exact}$\uparrow$  & \textsc{BLEU}$\uparrow$  & \textsc{Levenshtein}$\downarrow$  & \textsc{RDK FTS}$\uparrow$  & \textsc{MACCS FTS}$\uparrow$ & \textsc{Morgan FTS}$\uparrow$ & \textsc{Validity}$\uparrow$ \\
\midrule 
\rowcolor[RGB]{234, 238, 234}
& \multicolumn{8}{l}{\textit{Description-guided Molecule Design}} \\
\multirow{5}{*}{$^\clubsuit$} & \textsc{Alpaca} & 0.000 & 0.004 & 51.088 & 0.006 & 0.029 & 0.000 & 0.002 \\
& \textsc{Baize} & 0.000 & 0.006 & 53.796 & 0.000 & 0.000 & 0.000 & 0.002 \\
& \textsc{ChatGLM} & 0.000 & 0.004 & 53.157 & 0.005 & 0.000 & 0.000 & 0.005 \\
& \textsc{LLama} & 0.000 & 0.003 & 59.864 & 0.005 & 0.000 & 0.000 & 0.003 \\
& \textsc{Vicuna} & 0.000 & 0.006 & 60.356 & 0.006 & 0.001 & 0.000 & 0.001 \\
& \rebut{\textsc{Galactica}} & \rebut{0.000} & \rebut{0.192} & \rebut{44.152} & \rebut{0.135} & \rebut{0.248} & \rebut{0.088} & \rebut{0.992} \\
& \textbf{\textsc{Ours}} & \colorbox{babypink}{\tiny $\uparrow$0.002} \textbf{0.002} &  \colorbox{babypink}{\tiny $\uparrow$0.153} \textbf{0.345} &  \colorbox{babypink}{\tiny$\uparrow$2.785} \textbf{41.367} & \colorbox{babypink}{\tiny $\uparrow$0.096} \textbf{0.231} & \colorbox{babypink}{\tiny$\uparrow$0.164} \textbf{0.412} & \colorbox{babypink}{\tiny$\uparrow$0.059} \textbf{0.147} & \colorbox{babypink}{\tiny$\uparrow$0.008} \textbf{1.000} \\
\midrule
\multirow{2.5}{*}{$^\spadesuit$} & \rebut{\textsc{Text+Chem T5}} & \rebut{0.097} & \rebut{0.508} & \rebut{41.819} & \rebut{0.352} & \rebut{0.474} & \rebut{0.353} & \rebut{0.721} \\
& \rebut{\textsc{MolT5}} & \rebut{0.112} & \rebut{0.546} & \rebut{38.276} & \rebut{0.400} & \rebut{0.538} & \rebut{0.295} & \rebut{0.773} \\
% \midrule
% \midrule
% {\multirow{3}{*}{\textbf{Model}}} 
% & \multicolumn{7}{c}{\textbf{Reagent Prediction}} \\
% \cmidrule{2-8}
% & Exact $\uparrow$  & BLEU $\uparrow$  & Levenshtein $\downarrow$  & RDK FTS $\uparrow$  & MACCS FTS $\uparrow$ & Morgan FTS $\uparrow$ & Validity $\uparrow$ \\
\midrule[1.1pt]
\rowcolor[RGB]{234, 238, 234}
& \multicolumn{8}{l}{\textit{Reagent Prediction}} \\
\multirow{5}{*}{$^\clubsuit$} & \textsc{Alpaca} & 0.000 & 0.026 & 29.037 & 0.029 & 0.016 & 0.001 & 0.186 \\
& \textsc{Baize} & 0.000 & 0.051 & 30.628 & 0.022 & 0.018 & 0.004 & 0.099 \\
& \textsc{ChatGLM} & 0.000 & 0.019 & 29.169 & 0.017 & 0.006 & 0.002 & 0.074 \\
& \textsc{LLama} & 0.000 & 0.003 & 28.040 & 0.037 & 0.001 & 0.001 & 0.001 \\
& \textsc{Vicuna} & 0.000 & 0.010 & 27.948 & 0.038 & 0.002 & 0.001 & 0.007 \\
& \rebut{\textsc{Galactica}} & \rebut{0.000} & \rebut{0.141} & \rebut{30.760} & \rebut{0.036} & \rebut{0.127} & \rebut{0.051} & \rebut{0.995} \\
& \textbf{\textsc{Ours}} & \colorbox{babypink}{\tiny $\uparrow$0.044} \textbf{0.044} & \colorbox{babypink}{\tiny $\uparrow$0.083} \textbf{0.224} & \colorbox{babypink}{\tiny $\uparrow$4.781} \textbf{23.167} & \colorbox{babypink}{\tiny $\uparrow$0.200} \textbf{0.237} & \colorbox{babypink}{\tiny $\uparrow$0.237} \textbf{0.364} & \colorbox{babypink}{\tiny $\uparrow$0.162} \textbf{0.213} & \colorbox{babypink}{\tiny $\uparrow$0.005} \textbf{1.000} \\
\midrule
\multirow{1.5}{*}{$^\spadesuit$} & \rebut{\textsc{Text+Chem T5}} & \rebut{0.000} & \rebut{0.225} & \rebut{49.323} & \rebut{0.039} & \rebut{0.186} & \rebut{0.052} & \rebut{0.313} \\
% \midrule
% \midrule
% {\multirow{3}{*}{\textbf{Model}}} 
% & \multicolumn{7}{c}{\textbf{Forward Reaction Prediction}} \\
% \cmidrule{2-8}
% & Exact $\uparrow$  & BLEU $\uparrow$  & Levenshtein $\downarrow$  & RDK FTS $\uparrow$  & MACCS FTS $\uparrow$ & Morgan FTS $\uparrow$ & Validity $\uparrow$ \\
% \midrule 
\midrule[1.1pt]
\rowcolor[RGB]{234, 238, 234}
& \multicolumn{8}{l}{\textit{Forward Reaction Prediction}} \\
\multirow{5}{*}{$^\clubsuit$} & \textsc{Alpaca} & 0.000 & 0.065 & 41.989 & 0.004 & 0.024 & 0.008 & 0.138 \\
& \textsc{Baize} & 0.000 & 0.044 & 41.500 & 0.004 & 0.025 & 0.009 & 0.097 \\
& \textsc{ChatGLM} & 0.000 & 0.183 & 40.008 & 0.050 & 0.100 & 0.044 & 0.108 \\
& \textsc{LLama} & 0.000 & 0.020 & 42.002 & 0.001 & 0.002 & 0.001 & 0.039 \\
& \textsc{Vicuna} & 0.000 & 0.057 & 41.690 & 0.007 & 0.016 & 0.006 & 0.059 \\
& \rebut{\textsc{Galactica}} & \rebut{0.000} & \rebut{0.468} & \rebut{35.021} & \rebut{0.156} & \rebut{0.257} & \rebut{0.097} & \rebut{0.946} \\
& \textbf{\textsc{Ours}} & \colorbox{babypink}{\tiny $\uparrow$0.045} \textbf{0.045} &  \colorbox{babypink}{\tiny $\uparrow$0.186} \textbf{0.654} & \colorbox{babypink}{\tiny $\uparrow$7.759} \textbf{27.262} & \colorbox{babypink}{\tiny $\uparrow$0.157} \textbf{0.313} & \colorbox{babypink}{\tiny $\uparrow$0.252} \textbf{0.509} & \colorbox{babypink}{\tiny $\uparrow$0.165} \textbf{0.262} &  \colorbox{babypink}{\tiny $\uparrow$0.054} \textbf{1.000} \\
\midrule
\multirow{1.5}{*}{$^\spadesuit$} & \rebut{\textsc{Text+Chem T5}} & \rebut{0.239} & \rebut{0.782} & \rebut{20.413} & \rebut{0.705} & \rebut{0.789} & \rebut{0.652} & \rebut{0.762} \\
% \midrule
% \midrule
% {\multirow{3}{*}{\textbf{Model}}} 
% & \multicolumn{7}{c}{\textbf{Retrosynthesis}} \\
% \cmidrule{2-8}
% & Exact $\uparrow$  & BLEU $\uparrow$  & Levenshtein $\downarrow$  & RDK FTS $\uparrow$  & MACCS FTS $\uparrow$ & Morgan FTS $\uparrow$ & Validity $\uparrow$ \\
% \midrule 
\midrule[1.1pt]
\rowcolor[RGB]{234, 238, 234}
& \multicolumn{8}{l}{\textit{Retrosynthesis}} \\
\multirow{5}{*}{$^\clubsuit$} & \textsc{Alpaca} & 0.000 & 0.063 & 46.915 & 0.005 & 0.023 & 0.007 & 0.160 \\
& \textsc{Baize} & 0.000 & 0.095 & 44.714 & 0.025 & 0.050 & 0.023 & 0.112 \\
& \textsc{ChatGLM} & 0.000 & 0.117 & 48.365 & 0.056 & 0.075 & 0.043 & 0.046 \\
& \textsc{LLama} & 0.000 & 0.036 & 46.844 & 0.018 & 0.029 & 0.017 & 0.010 \\
& \textsc{Vicuna} & 0.000 & 0.057 & 46.877 & 0.025 & 0.030 & 0.021 & 0.017 \\
& \rebut{\textsc{Galactica}} & \rebut{0.000} & \rebut{0.452} & \rebut{34.940} & \rebut{0.167} & \rebut{0.274} & \rebut{0.134} & \rebut{0.986} \\
& \textbf{\textsc{Ours}} &  \colorbox{babypink}{\tiny $\uparrow$0.009} \textbf{0.009} & \colorbox{babypink}{\tiny $\uparrow$0.253} \textbf{0.705} & \colorbox{babypink}{\tiny $\uparrow$3.713} \textbf{31.227} & \colorbox{babypink}{\tiny $\uparrow$0.116} \textbf{0.283} & \colorbox{babypink}{\tiny $\uparrow$0.075} \textbf{0.487} & \colorbox{babypink}{\tiny $\uparrow$0.096} \textbf{0.230} & \colorbox{babypink}{\tiny $\uparrow$0.014} \textbf{1.000} \\
\midrule
\multirow{1.5}{*}{$^\spadesuit$} & \rebut{\textsc{Text+Chem T5}} & \rebut{0.141} & \rebut{0.765} & \rebut{24.043} & \rebut{0.685} & \rebut{0.765} & \rebut{0.585} & \rebut{0.698} \\
\bottomrule
\end{tabular}
}
\vskip -0.2in
\label{tab:design_reagent}
\end{table*}




==> tables/property.tex <==
\begin{wraptable}{l}{0.3\textwidth}
\centering
\vskip -0.3in
\small
\caption{\small
Results of molecular property prediction tasks.
}
\vskip 0.07in
\scalebox{0.9}{
\begin{tabular}{lccccccc}
\toprule
% {\multirow{3}{*}{\textsc{Model}}} 
% & \multicolumn{1}{c}{\textsc{Property Prediction}} \\
% \cmidrule(lr){2-2}
\textsc{Model}
&\textsc{MAE} $\downarrow$ \\
\midrule 
\rowcolor[RGB]{234, 238, 234}
\multicolumn{2}{l}{\textit{Property Prediction}} \\
\textsc{Alpaca} & 322.109\\
\textsc{Baize} & 261.343\\
\textsc{ChatGLM} & - \\
\textsc{LLama} & 5.553\\
\textsc{Vicuna} & 860.051 \\
\midrule
\textsc{Ours} & \colorbox{babypink}{\tiny$\uparrow$5.54} \textbf{0.013} \\
\bottomrule
\end{tabular}
}
\vskip -0.1in
\label{tab:moldes_prop}
\end{wraptable}

==> tables/protein_results.tex <==
\begin{table*}[!t]
\vskip -0.1in
\centering
\small
\caption{\small
Results for tasks related to protein understanding. These tasks encompass catalytic activity prediction, protein function prediction, domain/motif prediction and function description generation tasks.
}
\vskip 0.1in
\scalebox{0.8}{
\begin{tabular}{lcccc}
\toprule
{\multirow{3}{*}{\textsc{Model}}} 
& \multicolumn{1}{c}{\textsc{Protein Function}}
& \multicolumn{1}{c}{\textsc{Functional Description}} 
& \multicolumn{1}{c}{\textsc{Catalytic Activity}}
& \multicolumn{1}{c}{\textsc{Domain/Motif}}
\\
\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-4}
\cmidrule(lr){5-5}
% \toprule
% \textbf{Model} & \textbf{Protein Function} & \textbf{Functional Description} & \textbf{Catalytic Activity} & \textbf{Domain/Motif} \\
% \midrule 
& \textsc{ROUGE-L} $\uparrow$  & \textsc{ROUGE-L} $\uparrow$  & \textsc{ROUGE-L} $\uparrow$  & \textsc{ROUGE-L} $\uparrow$ \\
\midrule 
\textsc{Alpaca} & 0.20 & 0.10 & 0.23 & 0.12 \\
\textsc{Baize} &  0.20 & 0.15 & 0.22 & 0.13 \\
\textsc{ChatGLM} & 0.15 & 0.14 & 0.13 & 0.10 \\
\textsc{LLama} & 0.12 & 0.12 & 0.13 & 0.09 \\
\textsc{Vicuna} & 0.15 & 0.14 & 0.16 & 0.12 \\
\midrule
\textbf{Ours} & \textbf{0.42} & \textbf{0.44} &  \textbf{0.52} & \textbf{0.46} \\
\bottomrule
\end{tabular}
}
\label{tab:res_protein}
\end{table*}
